How to Train a (Bad) Algorithmic Caseworker: A Quantitative Deconstruction of Risk Assessments in Child-Welfare

Child welfare (CW) agencies use risk assessment tools as a means to achieve evidence-based, consistent, and unbiased decision-making. These risk assessments act as data collection mechanisms and have further evolved into algorithmic systems in recent years. Moreover, several of these algorithms have reinforced biased theoretical constructs and predictors because of the easy availability of structured assessment data. In this study, we critically examine the Washington Assessment of Risk Model (WARM), a prominent risk assessment tool that has been adopted by over 30 states in the United States and has been repurposed into more complex algorithms. We compared WARM against the narrative coding of casenotes written by caseworkers who used WARM. We found significant discrepancies between the casenotes and WARM data where WARM scores did not not mirror caseworkers' notes about family risk. We provide the SIGCHI community with some initial findings from the quantitative de-construction of a child-welfare algorithm.

==> CHI LBW - Camera Ready [Two Column]/table1.tex <==
 \begin{table}
  \Small
  \label{tab:freq}
  \begin{tabular}{|>{\raggedright}p{4cm}|>{\raggedright}p{2cm}|>{\raggedright}p{2cm}|>{\raggedright}p{2cm}|>{\raggedright}p{2cm}|>{\raggedright\arraybackslash}p{2.8cm}|}
     \toprule
     Variable & Parameter Estimate & Confidence (2.5\%) & Confidence (97.5\%) & Standard Error & Odds Ratio\\
     \midrule
     (Intercept)&-6.1808 ***&-7.2682&-5.1757&0.5331&0.0021\\
     Stress of caretaker^1&0.3703 ***&0.2383&0.5041&0.0677&1.4481\\
     Cooperation with agency^1&0.4059 ***&0.2555&0.5609&0.0777&1.5006\\
     Frequency of abuse/neglect&0.3015 ***&0.1876&0.4155&0.058&1.3519\\
     Age of child&0.3146 ***&0.1747&0.4601&0.0727&1.3697\\
     Deviant arousal^1&-0.1329 **&-0.2189&-0.0495&0.0432&0.8755\\
     Dangerous acts&0.1707 **&0.0586&0.2818&0.0569&1.1862\\
     Social support for caretaker^1&-0.1764 **&-0.2966&-0.0608&0.0601&0.8383\\
     History of abuse or neglect as a child^1&-0.1423 **&-0.2441&-0.0427&0.0513&0.8674\\
     Extent of emotional harm exhibited by child&0.1409 **&0.0377&0.243&0.0523&1.1513\\
     History of domestic violence^2&0.1544 *&0.0275&0.2832&0.0651&1.167\\
     Cooperation with agency^2&-0.1536 *&-0.2871&-0.0217&0.0676&0.8576\\
     Attachment and bonding^2&0.1298 *&0.0089&0.2517&0.0618&1.1386\\
     Child’s role in family^1&0.1129 *&0.0043&0.2202&0.055&1.1195\\
     Substance abuse^1&-0.1034 *&-0.2052&-0.0042&0.0512&0.9018\\
     Extent of physical injury&0.1248 .&-0.255&0.0007&0.0651&0.8827\\
     Child is pressured to recant or deny abuse^1&0.1073 .&-0.0027&0.2172&0.056&1.1132\\
     Personal boundary issues^1&0.0956 .&-0.0045&0.1954&0.0509&1.1003\\
     Parenting skills^2&-0.1430 .&-0.2957&0.0045&0.0765&0.8668\\
     Recognition of problem^1&0.1404 .&-0.0146&0.2935&0.0784&1.1507\\
     Victimization of other children by caretaker^1&0.0880 .&-0.0101&0.1846&0.0496&1.092\\
     Recognition of problem^2&0.1318 .&-0.0159&0.2804&0.0754&1.1408\\
     Exploitation (nonsexual)&-0.0766 .&-0.1638&0.0089&0.044&0.9263\\
     Parenting skills^1&0.1356 .&-0.0217&0.2936&0.0803&1.1452\\
     Child is pressured to recant or deny abuse^2&-0.0998&-0.2196&0.0194&0.0609&0.905\\
     History of domestic violence^1&-0.0989&-0.2219&0.0224&0.0622&0.9059\\
     Fear of home or caretaker&-0.0895&-0.2121&0.0301&0.0617&0.9144\\
  \bottomrule
 \end{tabular}
 \caption{Significant Variables from Backward Feature Selection}
   \begin{tablenotes}
        \item [1]\^1 Caretaker 1, ^2 Caretaker 2
        \item[2] Denotations of significance (p-value): *** [0, 0.001], ** (0.001, 0.01], * (0.01, 0.05], . (0.05, 0.1]
        \item [3]
    \end{tablenotes}
 \end{table}

==> table1.tex <==
 \begin{table}
  \Small
  \label{tab:freq}
  \begin{tabular}{|>{\raggedright}p{4cm}|>{\raggedright}p{2cm}|>{\raggedright}p{2cm}|>{\raggedright}p{2cm}|>{\raggedright}p{2cm}|>{\raggedright\arraybackslash}p{2.8cm}|}
     \toprule
     Variable & Parameter Estimate & Confidence (2.5\%) & Confidence (97.5\%) & Standard Error & Odds Ratio\\
     \midrule
     (Intercept)&-6.1808 ***&-7.2682&-5.1757&0.5331&0.0021\\
     Stress of caretaker^1&0.3703 ***&0.2383&0.5041&0.0677&1.4481\\
     Cooperation with agency^1&0.4059 ***&0.2555&0.5609&0.0777&1.5006\\
     Frequency of abuse/neglect&0.3015 ***&0.1876&0.4155&0.058&1.3519\\
     Age of child&0.3146 ***&0.1747&0.4601&0.0727&1.3697\\
     Deviant arousal^1&-0.1329 **&-0.2189&-0.0495&0.0432&0.8755\\
     Dangerous acts&0.1707 **&0.0586&0.2818&0.0569&1.1862\\
     Social support for caretaker^1&-0.1764 **&-0.2966&-0.0608&0.0601&0.8383\\
     History of abuse or neglect as a child^1&-0.1423 **&-0.2441&-0.0427&0.0513&0.8674\\
     Extent of emotional harm exhibited by child&0.1409 **&0.0377&0.243&0.0523&1.1513\\
     History of domestic violence^2&0.1544 *&0.0275&0.2832&0.0651&1.167\\
     Cooperation with agency^2&-0.1536 *&-0.2871&-0.0217&0.0676&0.8576\\
     Attachment and bonding^2&0.1298 *&0.0089&0.2517&0.0618&1.1386\\
     Child’s role in family^1&0.1129 *&0.0043&0.2202&0.055&1.1195\\
     Substance abuse^1&-0.1034 *&-0.2052&-0.0042&0.0512&0.9018\\
     Extent of physical injury&0.1248 .&-0.255&0.0007&0.0651&0.8827\\
     Child is pressured to recant or deny abuse^1&0.1073 .&-0.0027&0.2172&0.056&1.1132\\
     Personal boundary issues^1&0.0956 .&-0.0045&0.1954&0.0509&1.1003\\
     Parenting skills^2&-0.1430 .&-0.2957&0.0045&0.0765&0.8668\\
     Recognition of problem^1&0.1404 .&-0.0146&0.2935&0.0784&1.1507\\
     Victimization of other children by caretaker^1&0.0880 .&-0.0101&0.1846&0.0496&1.092\\
     Recognition of problem^2&0.1318 .&-0.0159&0.2804&0.0754&1.1408\\
     Exploitation (nonsexual)&-0.0766 .&-0.1638&0.0089&0.044&0.9263\\
     Parenting skills^1&0.1356 .&-0.0217&0.2936&0.0803&1.1452\\
     Child is pressured to recant or deny abuse^2&-0.0998&-0.2196&0.0194&0.0609&0.905\\
     History of domestic violence^1&-0.0989&-0.2219&0.0224&0.0622&0.9059\\
     Fear of home or caretaker&-0.0895&-0.2121&0.0301&0.0617&0.9144\\
  \bottomrule
 \end{tabular}
 \caption{Significant Variables from Backward Feature Selection}
   \begin{tablenotes}
        \item [1]\^1 Caretaker 1, ^2 Caretaker 2
        \item[2] Denotations of significance (p-value): *** [0, 0.001], ** (0.001, 0.01], * (0.01, 0.05], . (0.05, 0.1]
        \item [3]
    \end{tablenotes}
 \end{table}
